DeepRT: A Soft Real Time Scheduler for Computer Vision Applications on the Edge

The ubiquity of smartphone cameras and IoT cameras, together with the recent boom of deep learning and deep neural networks, proliferate various computer vision driven mobile and IoT applications deployed on the edge. This paper focuses on applications which make soft real time requests to perform inference on their data - they desire prompt responses within designated deadlines, but occasional deadline misses are acceptable. Supporting soft real time applications on a multi-tenant edge server is not easy, since the requests sharing the limited GPU computing resources of an edge server interfere with each other. In order to tackle this problem, we comprehensively evaluate how latency and throughput respond to different GPU execution plans. Based on this analysis, we propose a GPU scheduler, DeepRT, which provides latency guarantee to the requests while maintaining high overall system throughput. The key component of DeepRT, DisBatcher, batches data from different requests as much as possible while it is proven to provide latency guarantee for requests admitted by an Admission Control Module. DeepRT also includes an Adaptation Module which tackles overruns. Our evaluation results show that DeepRT outperforms state-of-the-art works in terms of the number of deadline misses and throughput.

==> archi.tex <==
\section{{\name} Workflow}
\label{sec:workflow}


\ccomment{
\begin{figure}
  	\centering
  	\includegraphics[width=1\linewidth]{figures/workflow.pdf}
	\caption{{\name} System workflow.}
	\label{fig:wf}
	\vspace{-5mm}
\end{figure}}

In this part we present an overview of the whole system of {\name}, shown in Figure \ref{fig:overview}. {\name} is a system built on top of the scheduling scheme presented in the previous section, aiming at providing a soft real time inference service for CNN models on GPU.

First, {\name} has a Performance Profiler which performs offline performance analysis to obtain the execution times of batched job instances of different batch sizes and different categories. %of the execution of different batches of images with different types.
When a new request arrives at {\name}, {\name} first routes this pending request to a two-phase Admission Control Module where {\name} performs an admission control test to determine whether the pending request is  schedulable under current system workload, based on the data provided by the Performance Profiler. If the new request together with current workload is schedulable, {\name} begins the processing of this request by passing its frames to a DisBatcher, where the frames get   batched with frames from other requests and queued. Then, an EDF scheduler commands a Worker on GPU to start processing the job instances. We also have an Adaptation Module which monitors the performance of the Worker and feeds back online performance to the Performance Profiler, and adjusts the execution plan when necessary.

==> references.tex <==
\begin{thebibliography}{1}

@article{ferguson2014big,
  title={Big data from small data: data-sharing in the'long tail'of neuroscience},
  author={Ferguson, Adam R and Nielson, Jessica L and Cragin, Melissa H and Bandrowski, Anita E and Martone, Maryann E},
  journal={Nature neuroscience},
  volume={17},
  number={11},
  pages={1442--1447},
  year={2014},
  publisher={Nature Research}
}

@article{holdren2011mgi,
  title={Materials genome initiative for global competitiveness},
  author={Holdren, J.P.},
  journal={National Science and Technology Council OSTP},
  year={2011}
}

@inproceedings{nguyen20174ceed,
  title={4CeeD: Real-Time Data Acquisition and Analysis Framework for Material-related Cyber-Physical Environments},
  author={Nguyen, Phuong and others},
  booktitle={Proceedings of the 17th IEEE/ACM International Symposium on Cluster, Cloud and Grid Computing},
  pages={11--20},
  year={2017},
  organization={IEEE Press}
}

@inproceedings{nguyen2017monad,
  title={MONAD: Self-adaptive Micro-service Infrastructure for Heterogeneous Scientific Workflows},
  author={Nguyen, Phuong and Nahrstedt, Klara},
  booktitle={Autonomic Computing (ICAC), 2017 IEEE International Conference on},
  pages={187--196},
  year={2017},
  organization={IEEE}
}


@misc{4ceedsurvey2016,
  title = {User Study and Survey on Material-related Experiments},
  howpublished = "\url{http://hdl.handle.net/2142/94738}",
  year = {2016}, 
  note = "[Online; accessed November 30, 2016]"
}

@article{mclennan2010hubzero,
  title={HUBzero: a platform for dissemination and collaboration in computational science and engineering},
  author={McLennan, Michael and Kennell, Rick},
  journal={Computing in Science \& Engineering},
  volume={12},
  number={2},
  year={2010},
  publisher={IEEE}
}

@article{mayernik2012data,
  title={The data conservancy instance: Infrastructure and organizational services for research data curation},
  author={Mayernik, Matthew S and Choudhury, G Sayeed and DiLauro, Tim and Metsger, Elliot and Pralle, Barbara and Rippin, Mike and Duerr, Ruth},
  journal={D-Lib Magazine},
  volume={18},
  number={9/10},
  year={2012},
  publisher={Corporation for National Research Initiatives}
}

@inproceedings{tong2016hierarchical,
  title={A hierarchical edge cloud architecture for mobile computing},
  author={Tong, Liang and Li, Yong and Gao, Wei},
  booktitle={INFOCOM 2016-The 35th Annual IEEE International Conference on Computer Communications, IEEE},
  pages={1--9},
  year={2016},
  organization={IEEE}
}

@article{mach2017mobile,
  title={Mobile edge computing: A survey on architecture and computation offloading},
  author={Mach, Pavel and Becvar, Zdenek},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={19},
  number={3},
  pages={1628--1656},
  year={2017},
  publisher={IEEE}
}

@inproceedings{tan2017online,
  title={Online job dispatching and scheduling in edge-clouds},
  author={Tan, Haisheng and Han, Zhenhua and Li, Xiang-Yang and Lau, Francis CM},
  booktitle={INFOCOM 2017-IEEE Conference on Computer Communications, IEEE},
  pages={1--9},
  year={2017},
  organization={IEEE}
}

@inproceedings{wang2016reconciling,
  title={Reconciling task assignment and scheduling in mobile edge clouds},
  author={Wang, Lin and Jiao, Lei and Kliazovich, Dzmitry and Bouvry, Pascal},
  booktitle={Network Protocols (ICNP), 2016 IEEE 24th International Conference on},
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@inproceedings{nguyen2013agile,
  title={AGILE: Elastic Distributed Resource Scaling for Infrastructure-as-a-Service.},
  author={Nguyen, Hiep and Shen, Zhiming and Gu, Xiaohui and Subbiah, Sethuraman and Wilkes, John},
  booktitle={ICAC},
  volume={13},
  pages={69--82},
  year={2013}
}

@inproceedings{matsunaga2010use,
  title={On the use of machine learning to predict the time and resources consumed by applications},
  author={Matsunaga, Andr{\'e}a and Fortes, Jos{\'e} AB},
  booktitle={Proceedings of the 2010 10th IEEE/ACM International Conference on Cluster, Cloud and Grid Computing},
  pages={495--504},
  year={2010},
  organization={IEEE Computer Society}
}

@inproceedings{chiang2014matrix,
  title={Matrix: Achieving Predictable Virtual Machine Performance in the Clouds.},
  author={Chiang, Ron Chi-Lung and Hwang, Jinho and Huang, H Howie and Wood, Timothy},
  booktitle={ICAC},
  pages={45--56},
  year={2014}
}

\end{thebibliography}

==> sensecloud.tex <==
\section{sensecloud}
\label{sec:sensecloud}



==> senseloc.tex <==
\section{SenseLoc}


